UAV-AdNet: Unsupervised Anomaly Detection using Deep Neural Networks for Aerial Surveillance

Anomaly detection is a key goal of autonomous surveillance systems that should be able to alert unusual observations. In this paper, we propose a holistic anomaly detection system using deep neural networks for surveillance of critical infrastructures (e.g., airports, harbors, warehouses) using an unmanned aerial vehicle (UAV). First, we present a heuristic method for the explicit representation of spatial layouts of objects in bird-view images. Then, we propose a deep neural network architecture for unsupervised anomaly detection (UAV-AdNet), which is trained on environment representations and GPS labels of bird-view images jointly. Unlike studies in the literature, we combine GPS and image data to predict abnormal observations. We evaluate our model against several baselines on our aerial surveillance dataset and show that it performs better in scene reconstruction and several anomaly detection tasks. The codes, trained models, dataset, and video will be available at https://bozcani.github.io/uavadnet.

==> temp.tex <==
\subsection{Network Training Performance}

We calculate a mean squared error on difference between the input and reconstructed data and observed how it changes during training:
\begin{equation}
E_{train} = \frac{1}{N}\sum_{i}^N {(\mathbf{x}_i - \mathbf{\hat{x}}_i)^2},
\label{train_error_equation}
\end{equation}
where $\mathbf{x}_i$ is the $i^{th}$ input grid vector in the dataset which has $N$ number of samples, and $\mathbf{\hat{x}}_i$ is corresponding reconstructed grid vector for $x_i$.

We look training and validation loss separately for baselines. We observe that without copy-crop links (CVAE and VAE) have higher reconstruction error regardless of feeding gps inputs. Moreover, feeding gps data as input to the networks (UAV-AdNet) causes lower reconstructed error compared to the network (UAV-AdNet-wo-gps).
\begin{figure}[!hbt] 
\centerline{
\includegraphics[width=0.49\textwidth]{figures/error_vs_epoch.pdf}
}
\caption{Reconstruction error vs epochs plot during training. Solid and dashed lines indicates training and validation errors respectively. Black colored lines belongs to network architecture with gps input and copy-crop link for the grid inputs. Red colored lines belong to the network architecture without gps input and with copy-crop link for the grid inputs. }
\end{figure}





%Table
\begin{table}[hbt!]
\caption{Comparison with existing studies on Scene Modeling for robots. $V^{3d}$:3D points and image from RGBD sensors; $V^{2d}$: RGB image from on board camera; A: Audial from microphone; H: Haptic from sensors; O: Ontological knowledge entity for any type of modality; GPS: GPS data ; UGV: Unmanned Ground Vehicle; UAV: Unmanned Aerial Vehicle; n/a: Robot platform is not mentioned in original work. 
\label{tbl:comparison}}
\begin{center}
\footnotesize
\begin{tabular}{c|cccc}\hline
Study & Main Method & Data & Robot & Task \\  
 &  & Modality & Platform & Env. \\  \hline \hline


\cite{CelikkanatConceptWeb2014}  & MRF & V^{3d}, A, H & humanoid robot & indoor \\
\cite{anand2013contextually}  & MRF & V^{3d} & UGV & indoor \\
\cite{lin2013holistic} & MRF & V^{3d} & n/a & indoor \\

\cite{li2017context} & BN & O & underwater robot & underwater \\

\cite{joho2013nonparametric} & DB process & V^{3d} & service robot & indoor \\

\cite{mastrogiovanni2011robots} & PL & O & UGV & indoor \\

\cite{hwang2006ontology} & Ontology & O & n/a & indoor \\

\cite{saxena2014robobrain, tenorth2009knowrob} & Ontology & O & service robot & indoor \\

\cite{bozcan2019cosmo, bozcan2018missing} & BM & V^{3d} & humanoid robot& indoor \\

\hline
our & H, DNN & V^{2d}, GPS & UAV & outdoor  \\
method &&  &  &   \\
\hline

\end{tabular}
\end{center}

\end{table}








Firstly, we remove gps input layer from UAV-AdNet and train and test it with input grid vectors only. We call this model as UAV-AdNet-wo-gps. Secondly, we remove copy-crop links for grid input layer from UAV-AdNet and keep gps input layer. This network has type of conditional variational autoencoder (CVAE) where the model is conditioned on gps data. Lastly, we use regular Variation Autoencoder (VAE) by removing both copy-crop links for input layer and gps inputs. Baseline summaries can be shown in Table \ref{tbl:baselines} .

 \begin{table}[hbt]
\caption{Baseline architectures compared to proposed network UAV-AdNet. \label{tbl:baselines}}
\centering
\begin{tabular}{|ccc|}\hline                                                                 
Network  & Gps inputs  & Copy-crop links \\ \hline \hline
UAV-AdNet &  yes    &  yes \\ \hline
UAV-AdNet-wo-gps &  yes    &  no \\ \hline
CVAE &  yes    &  no \\ \hline
VAE &  no    &  no \\ \hline
\end{tabular}
\end{table}
 







\subsection{Anomaly Detection Task}
%Our model can find anomalies (i.e. suspicious existence of objects) in given environment. For testing, we prepared test data and split it into three categories that each has different anomaly scenarios. The first category includes anomalies which violates security rules of DeepTech Experimental Hub (such as a person at the forbidden area -back side of the building-, a car in front of exits etc.). The second category includes anomalies which are not parts of DeepTech Experimental Hub rules  but belong to public rules (such as a car at the bike road, person on the road). The third category includes anomalies which are not part of neither private nor public rules. Therefore, it is difficult to detect these cases since they are implicit and require long-term observation of the environment. Rare existence of objects belong to this category (such as human at the right side of the building, trucks at the parking area of the building etc.)

Our model can find anomalies (i.e. suspicious existence of objects) in given environment. For testing, we split test data into three categories that each has different anomaly scenarios. The first anomaly category (Scenario 1) includes anomalies which breaks specific rules related to interested surveillance area (e.g. a person at the forbidden zone). The second anomaly category (Scenario 2) consists of anomalies which breaks public rules and they are not directly related to private rules (e.g. a car at the bike road). The third anomaly category (Scenario 3) includes anomalies which do not break neither private or public rules. Although these cases do not break any rules, they may raise suspicion due to rare occurrence (e.g. a truck at car parking area). Qualitative examples are given in Figure \ref{fig:scenerios}

\begin{figure}[hbt] 
\centerline{
\includegraphics[width=0.49\textwidth]{figures/scenarios_compressed.pdf}
}
\caption{Example images for different anomaly scenarios. Red and blue rectangles show anomaly and normal objects respectively. The left image indicates a case breaking of private rules of the area (Scenario 1). Humans are not allowed to enter back side of the building. The middle image shows a case breaking of public rule (Scenario 2). Bikes are not allowed to use vehicle roads. Right image shows an example of rare observation of objects which may arise suspicions. Bikes are usually parked at the bike parking area instead of car park of the building.\label{fig:scenerios}}
\end{figure}



%area private rules (i.e. private rules of DeepTech Experimental Hub) such as a person at the forbidden area (e.g. back side of the building).

For testing Scenario 1, we choose test samples which include cases breaking private rules. Moreover, we create syntactic scene representations by adding objects randomly into ground truth input grid vectors to increase the size of test set. Objects are chosen and put in order to create scene representations which include private rules breaking cases. Same method is applied to create synthetic scene representations for Scenario 2 and 3.


%Next, we evaluate our model with Scenario 2. For this end, we use real and synthetic samples as well. Lastly, we use only real samples to test Scenario 3 since the model is supposed to find anomalies for undefined rules. Therefore, creating syntactic samples for Scenario 3 does not make sense since this type of anomalies may not be defined and recognized by human. %For all scenarios, we define accuracy as the percentage of objects correctly estimated with respect to the labeled objects in the test dataset.

For evaluating the performance of the methods, we use precision, recall and F1-score which are defined as follows:
%
\begin{eqnarray}
\textrm{Precision} & = & \frac{\textrm{TP}}{\textrm{TP}+\textrm{FP}},\\
\textrm{Recall} & = & \frac{\textrm{TP}}{\textrm{TP}+\textrm{FN}},\\
\textrm{F1-score} & = & 2\cdot \frac{\textrm{Precision}\cdot \textrm{Recall}}{\textrm{Precision} + \textrm{Recall}},
\end{eqnarray}
%
{\noindent}where TP, FP and FN stand for the number of true positives, false positives and false negatives, respectively. For anomaly detection task, we define TP as the number of grid cells that have value $0$ in reconstructed data correctly according to the ground truth sample; FP as the number of grid cells that the model set value $1$ but should have been $0$ according to the ground truth; TN as the number of grid cells that are set to $0$ correctly according to ground truth, and FN as the number of objects that the model is set to $0$, yet should have been $1$ according to the ground truth. We can formally define these as follows: 
%
\begin{eqnarray}
TP & = & \left\vert \{x: x\in {G^1} \land x\in {M^1}  \} \right\vert , \label{eqn:task2hypothesiseqns} \\
TN & = & \left\vert \{x: x\in {G^0} \land x\in {M^0}  \} \right\vert , \nonumber \\
FP & = & \left\vert \{x: x\in {G^0} \land x\in {M^1}  \} \right\vert , \nonumber \\
FN & = & \left\vert \{x: x\in {G^1} \land x\in {M^0}  \} \right\vert \nonumber ,
\end{eqnarray}
%
{\noindent}where $x$ is an instance of a reconstructed grid vector that indicates existence of an object; ${G^1}$ and ${G^0}$ are the sets of grid cells which have value $1$ and $0$ respectively in the ground truth sample; and ${M^1}$ and ${M^0}$ are the sets of grid cells which have value $1$ and $0$ respectively at the end of the model's reconstruction.


As shown in Table \ref{tbl:results}, proposed method performs better than baselines for all scenarios. For Scenerio 1, 

% \begin{table}[hbt]
%\caption{Baseline architectures compared to proposed network UAV-AdNet. %\label{tbl:results}}
%centering
%\begin{tabular}{|cccc|}\hline                                                                 
%Network  & Scenerio 1  & Scenerio 2 & Scenerio 3 \\ \hline \hline
%UAV-AdNet &  \textbf{98.2\%}    &  \textbf{92.6\%} &  \textbf{81.7\%}  \\ \hline
%UAV-AdNet-wo-gps & 86.8 \% & 81.0\% & 75.3\% \\ \hline
%CVAE & 69.2\%    & 61.3\% & 57.2\%\\ \hline
%VAE &  67.1\%    & 61.3\% & 56.7\%\\ \hline
%\end{tabular}
%\end{table}

\begin{table}[hbt]
\caption{Scenerio 1 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9816}	& \textbf{1.0}   & \textbf{0.9907}   \\ 
UAV-AdNet-wo-gps & 0.9427 & 0.9984  &  0.9697  \\ 
CVAE & 0.1963 & 0.5165  &  0.2845   \\ 
VAE  & 0.1920	 &  0.4102   &  0.2616 \\ \hline
  
\end{tabular}
\end{table}


\begin{table}[hbt]
\caption{Scenerio 2 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9724}	& \textbf{0.9899}   & \textbf{0.9811}   \\ 
UAV-AdNet-wo-gps & 0.9621 & 0.99  &  0.9759  \\ 
cVAE & 0.1982 & 0.3955  &  0.2641   \\ 
VAE  & 0.1979	 &  0.3992   &  0.2646 \\ \hline
  
\end{tabular}
\end{table}

\begin{table}[hbt]
\caption{Scenerio 3 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9630}	& \textbf{0.9939}   & \textbf{0.9782}   \\ 
UAV-AdNet-wo-gps & 0.9517 & 0.9939  &  0.9723  \\ 
cVAE & 0.1958 & 0.5158  &  0.2839   \\ 
VAE  & 0.1990	 &  0.4113   &  0.2682 \\ \hline
  
\end{tabular}
\end{table}


\begin{table}[hbt]
\caption{Anomaly detection accuracy. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Scenario 1}  & \textbf{Scenario 2}  & \textbf{Scenario 3}  \\ \hline \hline
UAV-AdNet & \textbf{0.9214}	& \textbf{0.8614}   & \textbf{0.8255}   \\ 
UAV-AdNet-wo-gps & 0.8778 & 0.7912  &  0.7778  \\ 
cVAE & 0.6212 & 0.4413  &  0.4433   \\ 
VAE  & 0.6198	 &  0.4165   &  0.42 \\ \hline
  
\end{tabular}
\end{table}




%abstract
In this paper, we present a variant of deep neural networks (UAV-AdNet) which is trained in unsupervised manner for autonomous anomaly detection using UAVs. For this end, firstly, we propose grid-wise environment representation of bird-view images captured by UAVs. Secondly, we propose ..., a variant of VAE, that learns joint distribution of grid-wise scene representation of aerial images and corresponding gps labels recorded by the UAVs. We evaluate our model against several baselines on a aerial surveillance dataset, and show that it performs better in anomaly detection task.


% AE figure
\begin{figure} 
\centerline{
\includegraphics[width=0.49\textwidth]{figures/all_ae.pdf}
}
\caption{A schematic comparison neural network structures of AE (top) and VAE (bottom). White nodes indicates input neurons which takes input vector $\mathbf{x}$ consisting of 4 features and light gray nodes indicates output neurons representing output vector $\mathbf{\hat{x}}$. Dark gray nodes indicates hidden neurons of the network. AE encodes input $\mathbf{x}$ to a latent vector $\mathbf{h}$ which has size 2. VAE learns parameters ($\boldsymbol{\mu}, \boldsymbol{\sigma}$) of the probability distribution of input data representation. A vector $\mathbf{z}$ is sampled from the probability distribution that has parameters $\boldsymbol{\mu}$ and $\boldsymbol{\sigma}$. Then, output vector $\mathbf{\hat{x}}$ is reconstructed from $\mathbf{z}$.   \label{fig:all_ae}}
\end{figure}


\begin{figure}
\centerline{
	\subfigure[]{
 
    	\includegraphics[width=0.49\textwidth]{figures/autoencoder.pdf}
    }
}
\centerline{
	\subfigure[]{
    	\includegraphics[width=0.49\textwidth]{figures/variationalautoencoder.pdf}
    }
}
\caption{A schematic comparison neural network structures of AE (top) and VAE (bottom). White nodes indicates input neurons which takes input vector $\mathbf{x}$ consisting of 4 features and light gray nodes indicates output neurons representing output vector $\mathbf{\hat{x}}$. Dark gray nodes indicates hidden neurons of the network. AE encodes input $\mathbf{x}$ to a latent vector $\mathbf{h}$ which has size 2. VAE learns parameters ($\boldsymbol{\mu}, \boldsymbol{\sigma}$) of the probability distribution of input data representation. A vector $\mathbf{z}$ is sampled from the probability distribution that has parameters $\boldsymbol{\mu}$ and $\boldsymbol{\sigma}$. Then, output vector $\mathbf{\hat{x}}$ is reconstructed from $\mathbf{z}$.   \label{fig:all_ae}}
\end{figure}

Comparison of model architectures is given in Table \ref{tbl:baselines}. 
\begin{table}[hbt]
\caption{Baseline architectures compared to proposed network UAV-AdNet. \label{tbl:baselines}}
\centering
\begin{tabular}{|ccc|}\hline                                                                 
Network  & Gps inputs  & Copy-crop links \\ \hline \hline
UAV-AdNet &  yes    &  yes \\ \hline
UAV-AdNet-wo-gps &  yes    &  no \\ \hline
CVAE &  yes    &  no \\ \hline
VAE &  no    &  no \\ \hline
\end{tabular}
\end{table}






We can formally define these as follows: 
%
\begin{eqnarray}
TP & = & \left\vert \{x: x\in {G^1} \land x\in {M^1}  \} \right\vert , \label{eqn:task2hypothesiseqns} \\
TN & = & \left\vert \{x: x\in {G^0} \land x\in {M^0}  \} \right\vert ,  \\
FP & = & \left\vert \{x: x\in {G^0} \land x\in {M^1}  \} \right\vert ,  \\
FN & = & \left\vert \{x: x\in {G^1} \land x\in {M^0}  \} \right\vert  ,
\end{eqnarray}
%
{\noindent}where $x$ is an instance of a reconstructed grid vector that indicates the existence of an object; ${G^1}$ and ${G^0}$ are the sets of grid cells which have value $1$ and $0$ respectively in the ground truth sample; and ${M^1}$ and ${M^0}$ are the sets of grid cells which have value $1$ and $0$ respectively at the end of the model's reconstruction.





\subsection{Variational Autoencoders (VAEs)}
Although AEs can learn latent representation of the input data, latent vectors may be discontinuous in latent space. In that case, the network learns only encoding and reconstruction of the input data without learning any parameters of a probability distribution representing the data. Therefore, regular AE cannot model the data.

Variational Autoencoders (VAE) are variants of AE that can model the input data by having continuous latent space. In VAE, the encoder part encodes input ($\mathbf{x}$) to two different types of latent vectors: (i) mean vector $\mathbf{\mu}$ and (ii) variance vector $\mathbf{\sigma}$ corresponding to the mean and variance of the input data distribution respectively. During the training phase, the network learns these parameters of the probability distribution representing the data instead of just compressed representation (i.e., $\mathbf{h}$ in Eq. \ref{eqn:ae_f}). 

In order the network to have continuous latent space, a regularizer term is added to loss function which constrains the network to learn $\boldsymbol{\mu}, \boldsymbol{\sigma}$. Loss function for VAE can be defined as follows:
\begin{equation}
\mathcal{L} = \mathcal{L}_{rec}(\mathbf{x}, \mathbf{\hat{x}}) + \mathcal{L}_{reg},   
\end{equation}
where $\mathcal{L}_{rec}$ is same in Eq. \ref{eqn:ae_loss} and $\mathcal{L}_{reg}$ is the regularizer term which penalizes the network for having latent vectors $\boldsymbol{\mu}, \boldsymbol{\sigma}$ for being dissimilar from parameters of a prior data distribution $p(\mathbf{z})$. The overall loss function can be re-written as follows:
\begin{equation}
\mathcal{L} = \mathcal{L}_{rec}(\mathbf{x}, \mathbf{\hat{x}}) + \mathfrak{D}_\text{KL}[q(\boldsymbol{\mu}, \boldsymbol{\sigma} | \mathbf{x})\mid\mid p(\mathbf{z})],   
\end{equation}
where $\mathfrak{D}_\text{KL}$ is the Kullback-Leibler divergence (KL divergence) which measures discrepancy between two probability distribution and $q(\boldsymbol{\mu}, \boldsymbol{\sigma})$ is the probability distribution which is represented by model parameters $\boldsymbol{\mu}, \boldsymbol{\sigma}$ for given $\mathbf{x}$.











\section{BACKGROUND}
In this section, we will describe autoencoders and their variants (variational autoencoders and conditional autoencoders)
that are essential for us to be able to describe our proposed method and baseline models for comparison.

\subsection{Autoencoders (AEs)}
Autoencoders are variants of artificial neural networks that are used to encode data for dimensionality reduction in an unsupervised manner. Having less number of hidden neurons compared to input neurons, the architecture of AE imposes bottleneck in the network which forces an encoded representation of the original input. The encoder part learns the encoding of the input data using hidden neurons, and the decoder part learns the reconstruction of original input from encoded representation. 

The encoder part can be formulated as follows:
\begin{equation}
      f_{\theta}(\mathbf{x}) = \mathbf{h},  \label{eqn:ae_f}
\end{equation}
where $f$ is a neural network with parameters $\theta$ that approximates mapping from the input $\mathbf{x}$ to latent space representation $\mathbf{h}$. Similarly, the decoder part can be formulated as follows:
\begin{equation}
      g_{\omega}(\mathbf{h}) = \mathbf{\hat{x}},  
\end{equation}
where $g$ is a neural network with parameters $\omega$ that approximates mapping from the latent representation $\mathbf{h}$ to reconstructed data $\mathbf{\hat{x}}$. 

Training an AE minimizes the following reconstruction loss function:
\begin{equation}
    \mathcal{L}_{rec}(\mathbf{x}, \mathbf{\hat{x}}), \label{eqn:ae_loss}
\end{equation}{}
which penalizes the network for having dissimilar output $\mathbf{\hat{x}}$ from the original input $\mathbf{x}$ (e.g. mean square error, cross entropy error).











\subsection{Variational Autoencoders (VAEs)}
Although AEs can learn latent representation of the input data, latent vectors may be discontinuous in latent space. In that case, the network learns only encoding and reconstruction of the input data without learning any parameters of a probability distribution representing the data. Therefore, regular AE cannot model the data.

Variational Autoencoders (VAE) are variants of AE that can model the input data by having continuous latent space. In VAE, the encoder part encodes input ($\mathbf{x}$) to two different types of latent vectors: (i) mean vector $\mathbf{\mu}$ and (ii) variance vector $\mathbf{\sigma}$ corresponding to the mean and variance of the input data distribution respectively. During the training phase, the network learns these parameters of the probability distribution representing the data instead of just compressed representation, i.e., $\mathbf{h}$ in (\ref{eqn:ae_f}). 

In order the network to have continuous latent space, a regularizer term is added to loss function which constrains the network to learn $\boldsymbol{\mu}, \boldsymbol{\sigma}$. The overall loss function for VAE can be defined as follows:
\begin{equation}
\mathcal{L} = {\mathcal{L}_{rec}}(\mathbf{x}, \mathbf{\hat{x}}) + {\mathfrak{D}_\text{KL}}[q(\boldsymbol{\mu}, \boldsymbol{\sigma} \mid \mathbf{x})\mid\mid p(\mathbf{z})],   
\end{equation}

where $\mathcal{L}_{rec}$ is same in (\ref{eqn:ae_loss}) and $\mathfrak{D}_\text{KL}$ is the Kullback-Leibler divergence which measures the discrepancy between two probability distribution and $q(\boldsymbol{\mu}, \boldsymbol{\sigma})$ is the probability distribution which is represented by model parameters $\boldsymbol{\mu}, \boldsymbol{\sigma}$ for given $\mathbf{x}$.




